Partial identification of kernel based two sample tests with mismeasured data

Nonparametric two-sample tests such as the Maximum Mean Discrepancy (MMD) are often used to detect differences between two distributions in machine learning applications. However, the majority of existing literature assumes that error-free samples from the two distributions of interest are available.We relax this assumption and study the estimation of the MMD under $\epsilon$-contamination, where a possibly non-random $\epsilon$ proportion of one distribution is erroneously grouped with the other. We show that under $\epsilon$-contamination, the typical estimate of the MMD is unreliable. Instead, we study partial identification of the MMD, and characterize sharp upper and lower bounds that contain the true, unknown MMD. We propose a method to estimate these bounds, and show that it gives estimates that converge to the sharpest possible bounds on the MMD as sample size increases, with a convergence rate that is faster than alternative approaches. Using three datasets, we empirically validate that our approach is superior to the alternatives: it gives tight bounds with a low false coverage rate.

==> tables.tex <==
\begin{table}[H] \label{MIMIC_FOREST_2k}
\caption{2000 Samples random contaminations}
$\epsilon = 0.1$ \\
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ll|ll|ll|}
\toprule
          & \multicolumn{2}{c|}{MIMIC ($n = 2000, d = 2)$} & \multicolumn{2}{c|}{FOREST $(n = 2000, d = 54)$} & \multicolumn{2}{c|}{BIO $(n = 72, d = 7128)$} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
Approach  & FCR    & MIW   & FCR    & MIW & FCR    & MIW    \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
S-SD (Ours)     & $0.0 \pm (0.0)$ & $0.154 \pm (0.001)$  & $0.0 \pm (0.0)$ & $0.049 \pm (0.001)$  & $0.01 \pm (0.01)$ & $0.043 \pm (0.001)$ \\
S-QNO      & $0.0 \pm (0.0)$ & $0.146 \pm (0.001)$ &  $0.0 \pm (0.0)$ & $0.047 \pm (0.001)$  & $1.0 \pm (0.0)$ & $0.028 \pm (0.0)$ \\
QNO               & $0.0 \pm (0.0)$ & $0.147 \pm (0.001)$ & $0.02 \pm (0.02)$ & $0.035 \pm (0.001)$  & $1.0 \pm (0.0)$ & $0.027 \pm (0.0)$ \\
SD                & $0.0 \pm (0.0)$ & $0.152 \pm (0.001)$ & $0.12 \pm (0.046)$ & $0.038 \pm (0.001)$  & $0.01 \pm (0.01)$ & $0.042 \pm (0.001)$ \\
SM                & $0.0 \pm (0.0)$ & $0.148 \pm (0.001)$ & $0.12 \pm (0.046)$ & $0.037 \pm (0.001)$  & $0.12 \pm (0.032)$ & $0.033 \pm (0.001)$ \\
Bootstrap        & $0.56 \pm (0.07)$ & $0.029 \pm (0.001)$ & $0.08 \pm (0.038)$ & $0.007 \pm (0.0)$   & $0.0 \pm (0.0)$ & $0.056 \pm (0.001)$ \\
\bottomrule 
\end{tabular}}
\\ \rule{0pt}{2ex} 

$\epsilon = 0.2$ \\
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ll|ll|ll|}
\toprule
          & \multicolumn{2}{c|}{MIMIC ($n = 2000, d = 2)$} & \multicolumn{2}{c|}{FOREST $(n = 2000, d = 54)$} & \multicolumn{2}{c|}{BIO $(n = 72, d = 7128)$} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
Approach  & FCR    & MIW   & FCR    & MIW & FCR    & MIW    \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
S-SD (Ours)    & $0.0 \pm (0.0)$ & $0.258 \pm (0.002)$  & $0.0 \pm (0.0)$ & $0.107 \pm (0.002)$  & $0.07 \pm (0.026)$ & $0.08 \pm (0.001)$ \\
S-QNO    & $0.0 \pm (0.0)$ & $0.258 \pm (0.002)$  & $0.0 \pm (0.0)$ & $0.114 \pm (0.002)$   & $1.0 \pm (0.0)$ & $0.056 \pm (0.001)$ \\
QNO               & $0.0 \pm (0.0)$ & $0.247 \pm (0.002)$  & $0.4 \pm (0.069)$ & $0.051 \pm (0.002)$  & $1.0 \pm (0.0)$ & $0.038 \pm (0.001)$ \\
SD                & $0.0 \pm (0.0)$ & $0.24 \pm (0.002)$  & $0.92 \pm (0.038)$ & $0.064 \pm (0.003)$  & $0.15 \pm (0.036)$ & $0.074 \pm (0.001)$ \\
SM               & $0.0 \pm (0.0)$ & $0.225 \pm (0.002)$  & $0.92 \pm (0.038)$ & $0.06 \pm (0.003)$   & $0.42 \pm (0.049)$ & $0.05 \pm (0.002)$ \\
Bootstrap       & $1.0 \pm (0.0)$ & $0.02 \pm (0.0)$    & $0.6 \pm (0.069)$ & $0.005 \pm (0.0)$  & $0.85 \pm (0.036)$ & $0.036 \pm (0.001)$ \\
\bottomrule
\end{tabular}}
\\ \rule{0pt}{2ex} 

$\epsilon = 0.3$  \\
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ll|ll|ll|}
\toprule
          & \multicolumn{2}{c|}{MIMIC ($n = 2000, d = 2)$} & \multicolumn{2}{c|}{FOREST $(n = 2000, d = 54)$} & \multicolumn{2}{c|}{BIO $(n = 72, d = 7128)$} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
Approach  & FCR    & MIW   & FCR    & MIW & FCR    & MIW    \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
S-SD (Ours)      & $0.0 \pm (0.0)$ & $0.331 \pm (0.002)$  & $0.0 \pm (0.0)$ & $0.168 \pm (0.002)$   & $0.12 \pm (0.032)$ & $0.096 \pm (0.001)$ \\
S-QNO     & $0.0 \pm (0.0)$ & $0.365 \pm (0.002)$   & $0.0 \pm (0.0)$ & $0.194 \pm (0.003)$   & $1.0 \pm (0.0)$ & $0.071 \pm (0.001)$ \\
QNO             & $0.0 \pm (0.0)$ & $0.329 \pm (0.002)$    & $0.96 \pm (0.028)$ & $0.073 \pm (0.002)$  & $1.0 \pm (0.0)$ & $0.032 \pm (0.001)$ \\
SD              & $0.0 \pm (0.0)$ & $0.267 \pm (0.003)$    & $1.0 \pm (0.0)$ & $0.077 \pm (0.004)$  & $0.42 \pm (0.049)$ & $0.085 \pm (0.002)$ \\
SM               & $0.0 \pm (0.0)$ & $0.242 \pm (0.002)$   & $1.0 \pm (0.0)$ & $0.068 \pm (0.003)$  & $0.57 \pm (0.05)$ & $0.059 \pm (0.002)$ \\
Bootstrap         & $1.0 \pm (0.0)$ & $0.015 \pm (0.0)$    & $0.86 \pm (0.049)$ & $0.003 \pm (0.0)$  & $1.0 \pm (0.0)$ & $0.027 \pm (0.0)$ \\
\bottomrule 
\end{tabular}}
\\ \rule{0pt}{2ex} 

$\epsilon = 0.4$  \\
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ll|ll|ll|}
\toprule
          & \multicolumn{2}{c|}{MIMIC ($n = 2000, d = 2)$} & \multicolumn{2}{c|}{FOREST $(n = 2000, d = 54)$} & \multicolumn{2}{c|}{BIO $(n = 72, d = 7128)$} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
Approach  & FCR    & MIW   & FCR    & MIW & FCR    & MIW    \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
S-SD (Ours)     & $0.0 \pm (0.0)$ & $0.394 \pm (0.002)$  & $0.0 \pm (0.0)$ & $0.237 \pm (0.003)$  & $0.17 \pm (0.038)$ & $0.108 \pm (0.001)$ \\
S-QNO   & $0.0 \pm (0.0)$ & $0.48 \pm (0.003)$   & $0.0 \pm (0.0)$ & $0.288 \pm (0.003)$  & $1.0 \pm (0.0)$ & $0.093 \pm (0.001)$ \\
QNO             & $0.0 \pm (0.0)$ & $0.427 \pm (0.002)$ & $0.98 \pm (0.02)$ & $0.08 \pm (0.002)$  & $1.0 \pm (0.0)$ & $0.023 \pm (0.001)$ \\
SD              & $0.9 \pm (0.042)$ & $0.265 \pm (0.004)$  & $1.0 \pm (0.0)$ & $0.085 \pm (0.004)$  & $0.52 \pm (0.05)$ & $0.093 \pm (0.002)$ \\
SM              & $0.9 \pm (0.042)$ & $0.231 \pm (0.003)$ & $1.0 \pm (0.0)$ & $0.071 \pm (0.003)$  & $0.6 \pm (0.049)$ & $0.068 \pm (0.002)$ \\
Bootstrap        & $1.0 \pm (0.0)$ & $0.012 \pm (0.0)$   & $0.98 \pm (0.02)$ & $0.003 \pm (0.0)$  & $1.0 \pm (0.0)$ & $0.018 \pm (0.0)$ \\
\bottomrule
\end{tabular}}
\\ \rule{0pt}{2ex} 

$\epsilon = 0.7$  \\
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ll|ll|ll|}
\toprule
          & \multicolumn{2}{c|}{MIMIC ($n = 2000, d = 2)$} & \multicolumn{2}{c|}{FOREST $(n = 2000, d = 54)$} & \multicolumn{2}{c|}{BIO $(n = 72, d = 7128)$} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
Approach  & FCR    & MIW   & FCR    & MIW & FCR    & MIW    \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
S-SD (Ours)      & $0.0 \pm (0.0)$ & $0.525 \pm (0.002)$  & $0.0 \pm (0.0)$ & $0.396 \pm (0.003)$  & $0.42 \pm (0.049)$ & $0.117 \pm (0.002)$ \\
Ours - S-QNO   & $0.0 \pm (0.0)$ & $0.83 \pm (0.005)$    & $0.0 \pm (0.0)$ & $0.559 \pm (0.004)$  & $1.0 \pm (0.0)$ & $0.113 \pm (0.002)$ \\
QNO            & $0.0 \pm (0.0)$ & $0.722 \pm (0.003)$   & $1.0 \pm (0.0)$ & $0.031 \pm (0.001)$ & $1.0 \pm (0.0)$ & $0.008 \pm (0.001)$ \\
SD              & $1.0 \pm (0.0)$ & $0.141 \pm (0.004)$ & $1.0 \pm (0.0)$ & $0.052 \pm (0.005)$ & $0.62 \pm (0.049)$ & $0.091 \pm (0.002)$ \\
SM            & $1.0 \pm (0.0)$ & $0.109 \pm (0.003)$   & $1.0 \pm (0.0)$ & $0.035 \pm (0.004)$  & $0.68 \pm (0.047)$ & $0.088 \pm (0.002)$ \\
Bootstrap      & $1.0 \pm (0.0)$ & $0.005 \pm (0.0)$    & $0.98 \pm (0.02)$ & $0.001 \pm (0.0)$   & $1.0 \pm (0.0)$ & $0.007 \pm (0.0)$ \\
\bottomrule
\end{tabular}}
\end{table}




\begin{table}[H] \label{MIMIC_FOREST_2k}
\caption{100 Samples nonrandom contaminations}
$\epsilon = 0.1$ \\
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ll|ll|ll|}
\toprule
          & \multicolumn{2}{c|}{MIMIC ($n = 100, d = 2)$} & \multicolumn{2}{c|}{FOREST $(n = 100, d = 54)$} & \multicolumn{2}{c|}{BIO $(n = 72, d = 7128)$} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
Approach  & FCR    & MIW   & FCR    & MIW & FCR    & MIW    \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
S-SD (Ours)       & $0.0 \pm (0.0)$ & $0.111 \pm (0.006)$        & $0.12 \pm (0.046)$ & $0.035 \pm (0.001)$    & $0.04 \pm (0.02)$ & $0.038 \pm (0.001)$ \\
Ours - S-QNO      & $0.96 \pm (0.028)$ & $0.095 \pm (0.005)$     & $0.26 \pm (0.062)$ & $0.036 \pm (0.001)$    & $1.0 \pm (0.0)$ & $0.027 \pm (0.0)$ \\
QNO               & $0.92 \pm (0.038)$ & $0.096 \pm (0.005)$     & $0.52 \pm (0.071)$ & $0.019 \pm (0.002)$    & $1.0 \pm (0.0)$ & $0.024 \pm (0.0)$ \\
SD               & $0.64 \pm (0.068)$ & $0.106 \pm (0.007)$      & $0.6 \pm (0.069)$ & $0.021 \pm (0.002)$      & $0.04 \pm (0.02)$ & $0.037 \pm (0.001)$ \\
SM                 & $0.68 \pm (0.066)$ & $0.104 \pm (0.006)$    & $0.58 \pm (0.07)$ & $0.021 \pm (0.002)$     & $0.67 \pm (0.047)$ & $0.023 \pm (0.001)$ \\
Bootstrap         & $0.48 \pm (0.071)$ & $0.098 \pm (0.005)$     & $0.18 \pm (0.054)$ & $0.038 \pm (0.001)$     & $0.52 \pm (0.068)$ & $0.054 \pm (0.001)$ \\
\bottomrule
\end{tabular}}
\\ \rule{0pt}{2ex} 

$\epsilon = 0.2$ \\
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ll|ll|ll|}
\toprule
          & \multicolumn{2}{c|}{MIMIC ($n = 100, d = 2)$} & \multicolumn{2}{c|}{FOREST $(n = 100, d = 54)$} & \multicolumn{2}{c|}{BIO $(n = 72, d = 7128)$} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
Approach  & FCR    & MIW   & FCR    & MIW & FCR    & MIW    \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
Ours - S-SD      & $\mathbf{0.0 \pm (0.0)}$ & $\mathbf{0.137 \pm (0.008)}$      & $\mathbf{0.0 \pm (0.0)}$ & $\mathbf{0.088 \pm (0.003)}$     & $\mathbf{0.1 \pm (0.03)}$ & $\mathbf{0.075 \pm (0.001)}$ \\
S-SD (Ours)      & $0.08 \pm (0.067)$ & $0.119 \pm (0.006)$   & $0.02 \pm (0.02)$ & $0.084 \pm (0.004)$     & $1.0 \pm (0.0)$ & $0.059 \pm (0.001)$ \\
QNO              & $0.58 \pm (0.069)$ & $0.13 \pm (0.006)$    & $0.62 \pm (0.069)$ & $0.033 \pm (0.006)$     & $1.0 \pm (0.0)$ & $0.037 \pm (0.001)$ \\
SD               & $0.64 \pm (0.068)$ & $0.082 \pm (0.01)$   & $0.9 \pm (0.042)$ & $0.027 \pm (0.005)$      & $0.13 \pm (0.034)$ & $0.069 \pm (0.001)$ \\
SM               & $0.66 \pm (0.067)$ & $0.08 \pm (0.01)$    & $0.9 \pm (0.042)$ & $0.026 \pm (0.004)$      & $0.82 \pm (0.038)$ & $0.037 \pm (0.001)$ \\
Bootstrap        & $0.94 \pm (0.034)$ & $0.048 \pm (0.002)$  & $0.4 \pm (0.069)$ & $0.034 \pm (0.001)$      & $0.25 \pm (0.043)$ & $0.036 \pm (0.001)$ \\
\bottomrule
\end{tabular}}
\\ \rule{0pt}{2ex} 

$\epsilon = 0.3$  \\
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ll|ll|ll|}
\toprule
          & \multicolumn{2}{c|}{MIMIC ($n = 100, d = 2)$} & \multicolumn{2}{c|}{FOREST $(n = 100, d = 54)$} & \multicolumn{2}{c|}{BIO $(n = 72, d = 7128)$} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
Approach  & FCR    & MIW   & FCR    & MIW & FCR    & MIW    \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
S-SD (Ours)     & $0.0 \pm (0.0)$ & $0.212 \pm (0.008)$     & $0.0 \pm (0.0)$ & $0.159 \pm (0.006)$     & $0.1 \pm (0.03)$ & $0.092 \pm (0.001)$ \\
S-QNO    & $0.16 \pm (0.052)$ & $0.248 \pm (0.011)$  & $0.0 \pm (0.0)$ & $0.159 \pm (0.007)$      & $0.94 \pm (0.024)$ & $0.076 \pm (0.001)$ \\
QNO             & $0.04 \pm (0.028)$ & $0.209 \pm (0.006)$  & $0.56 \pm (0.07)$ & $0.138 \pm (0.015)$     & $1.0 \pm (0.0)$ & $0.036 \pm (0.001)$ \\
SD              & $0.4 \pm (0.069)$ & $0.109 \pm (0.01)$    & $0.92 \pm (0.038)$ & $0.063 \pm (0.008)$      & $0.11 \pm (0.031)$ & $0.084 \pm (0.001)$ \\
SM              & $0.4 \pm (0.069)$ & $0.1 \pm (0.009)$     & $0.94 \pm (0.034)$ & $0.057 \pm (0.007)$     & $0.77 \pm (0.042)$ & $0.046 \pm (0.002)$ \\
Bootstrap       & $0.92 \pm (0.038)$ & $0.034 \pm (0.002)$  & $0.54 \pm (0.07)$ & $0.028 \pm (0.001)$       & $0.95 \pm (0.022)$ & $0.028 \pm (0.0)$ \\
\bottomrule
\end{tabular}}
\\ \rule{0pt}{2ex} 

$\epsilon = 0.4$  \\
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ll|ll|ll|}
\toprule
          & \multicolumn{2}{c|}{MIMIC ($n = 100, d = 2)$} & \multicolumn{2}{c|}{FOREST $(n = 100, d = 54)$} & \multicolumn{2}{c|}{BIO $(n = 72, d = 7128)$} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
Approach  & FCR    & MIW   & FCR    & MIW & FCR    & MIW    \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
S-SD (Ours)     & $0.0 \pm (0.0)$ & $0.312 \pm (0.007)$   & $0.0 \pm (0.0)$ & $0.211 \pm (0.006)$     & $0.16 \pm (0.037)$ & $0.109 \pm (0.001)$ \\
S-QNO   & $0.04 \pm (0.028)$ & $0.4 \pm (0.013)$  & $0.0 \pm (0.0)$ & $0.23 \pm (0.012)$     & $0.79 \pm (0.041)$ & $0.1 \pm (0.002)$ \\
QNO            & $0.0 \pm (0.0)$ & $0.299 \pm (0.008)$    & $0.62 \pm (0.069)$ & $0.226 \pm (0.019)$    & $1.0 \pm (0.0)$ & $0.028 \pm (0.001)$ \\
SD             & $0.6 \pm (0.069)$ & $0.151 \pm (0.012)$  & $0.96 \pm (0.028)$ & $0.053 \pm (0.011)$    & $0.22 \pm (0.041)$ & $0.098 \pm (0.001)$ \\
SM             & $0.6 \pm (0.069)$ & $0.13 \pm (0.01)$    & $0.96 \pm (0.028)$ & $0.045 \pm (0.009)$     & $0.69 \pm (0.046)$ & $0.061 \pm (0.002)$ \\
Bootstrap      & $0.9 \pm (0.042)$ & $0.03 \pm (0.002)$   & $0.58 \pm (0.07)$ & $0.021 \pm (0.001)$     & $1.0 \pm (0.0)$ & $0.019 \pm (0.0)$ \\
\bottomrule
\end{tabular}}
\\ \rule{0pt}{2ex} 

$\epsilon = 0.7$  \\
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ll|ll|ll|}
\toprule
          & \multicolumn{2}{c|}{MIMIC ($n = 100, d = 2)$} & \multicolumn{2}{c|}{FOREST $(n = 100, d = 54)$} & \multicolumn{2}{c|}{BIO $(n = 72, d = 7128)$} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
Approach  & FCR    & MIW   & FCR    & MIW & FCR    & MIW    \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
S-SD (Ours)     & $0.0 \pm (0.0)$ & $0.553 \pm (0.008)$     & $0.0 \pm (0.0)$ & $0.416 \pm (0.009)$     & $0.21 \pm (0.041)$ & $0.122 \pm (0.001)$ \\
S-QNO   & $0.0 \pm (0.0)$ & $0.755 \pm (0.025)$     & $0.0 \pm (0.0)$ & $0.568 \pm (0.026)$      & $0.89 \pm (0.049)$ & $0.12 \pm (0.002)$ \\
QNO            & $0.0 \pm (0.0)$ & $0.597 \pm (0.012)$     & $0.78 \pm (0.063)$ & $0.56 \pm (0.029)$    & $1.0 \pm (0.0)$ & $0.01 \pm (0.001)$ \\
SD             & $0.96 \pm (0.028)$ & $0.171 \pm (0.013)$  & $1.0 \pm (0.0)$ & $0.103 \pm (0.013)$       & $0.29 \pm (0.045)$ & $0.104 \pm (0.001)$ \\
SM             & $0.96 \pm (0.028)$ & $0.123 \pm (0.011)$   & $1.0 \pm (0.0)$ & $0.078 \pm (0.01)$      & $0.55 \pm (0.05)$ & $0.089 \pm (0.002)$ \\
Bootstrap      & $0.88 \pm (0.046)$ & $0.023 \pm (0.002)$   & $0.9 \pm (0.042)$ & $0.017 \pm (0.001)$    & $1.0 \pm (0.0)$ & $0.007 \pm (0.0)$ \\
\bottomrule
\end{tabular}}
\end{table}
